Collaborative Comic Generation: Integrating Visual Narrative Theories with AI Models for Enhanced Creativity

This study presents a theory-inspired visual narrative generative system that integrates conceptual principles-comic authoring idioms-with generative and language models to enhance the comic creation process. Our system combines human creativity with AI models to support parts of the generative process, providing a collaborative platform for creating comic content. These comic-authoring idioms, derived from prior human-created image sequences, serve as guidelines for crafting and refining storytelling. The system translates these principles into system layers that facilitate comic creation through sequential decision-making, addressing narrative elements such as panel composition, story tension changes, and panel transitions. Key contributions include integrating machine learning models into the human-AI cooperative comic generation process, deploying abstract narrative theories into AI-driven comic creation, and a customizable tool for narrative-driven image sequences. This approach improves narrative elements in generated image sequences and engages human creativity in an AI-generative process of comics. We open-source the code at https://github.com/RimiChen/Collaborative_Comic_Generation.

==> 0_0_Notes.tex <==
Key information to include:


1. **Overview of the Tool**:
    - Brief description of the tool's purpose and capabilities.
    - High-level architecture diagram to provide a visual summary.
2. **API Description**:
    - **Functionality**: List the primary functions offered by the API.
    - **Endpoints**: Detail the main endpoints, including their purpose, required parameters, and expected outputs.
    - **Examples**: Provide a few concise code examples demonstrating typical API usage.
3. **GUI Description**:
    - **Interface Elements**: Describe the key elements of the GUI, such as buttons, menus, and panels.
    - **User Workflow**: Explain how a user interacts with the interface to achieve common tasks.
    - **Screenshots**: Include annotated screenshots to visually represent the interface.
4. **Integration of API and GUI**:
    - Explain how the GUI interacts with the API to provide a seamless user experience.
5. **Evaluation and User Feedback**:
    - If space allows, briefly include any evaluation results or user feedback that highlights the effectiveness of the tool.




==> 2_RelatedWork.tex <==
%%% Related Work
%% Compare our tool to existing solutions, emphasizing unique features or improvements.

Narrative generation research and practice often separates out story plot specification from realization or telling\cite{chatman1980story}\cite{jhala2005discourse}. This allows researchers to separate out reasoning about plot structure and apply constraints on media selection to support the authorial goals with respect to the generated plots. Comics contain both visual media components and language components including stylized annotations and panel compositions. Comic artists have documented their process and principles from their experience. Eisner's book discusses the diversity of comics' image representations \cite{eisner2008comics}; Carrier et al.\cite{carrier2001aesthetics} provides a commentary on the aesthetics of comic strips as a form of fine art. Scott McCloud's work, which provides a comprehensive treatment of the many aspects of comic development, such as panel transitions that capture the focus changes between consecutive panels, the expression of action over time, and the symbolic metaphors that make abstract ideas visible \cite{mccloud1993understanding,mccloud1998understanding,mccloud2006making}. Besides the principles that apply to graphical aspects, the underlying structure of visual narrative has also received focus recently. Cohn et al.\cite{cohn2013visual,cohn2014grammar,cohn2015analyze,cohn2016visual} provide a comprehensive treatment of the cognitive processes from low-level perception through high-level discourse and organization\cite{freytag1908freytag,stern2000making,pratt2009narrative} with their proposed theory of the Visual Narrative Grammar (VNG).


Besides discussing comic structures and visual grammar,  other researchers have developed models or systems to generate sequential art that incorporates different features based on the analyzed theories and ideas. Alves et al.\cite{alvesgenerating} discussed the graphical composition of panels by describing the camera placement, background, independence, and other features. In comparison, Nairat et al.\cite{nairat2020generative} focus more on the fictional part of comic. They propose inner character evolutions to form stories which are then rendered as comics. Martens et al.\cite{martens2016discourse,martens2016generating} propose a visual narrative engine from the point of view of generative systems for the discourse of comic sequences. Their sample generator uses abstract shapes for demonstrating the variety of stories that can be communicated.

Our work aims to provide a generator that integrates and tests multiple aspects of comics rather than focusing on only one element to tackle the challenge result from the complexity of this visual medium. Our generator divides the complex generation problem by systematically organizing layers of decision making for composing comics. To achieve this, the generator supports the functions that can modify elements obtained from decomposing either comic's graphical composition and the structure as well as discourse elements, which makes the generator extendable and modular. We demonstrate how to encode concepts from a sample set of theories into the generator and provide sample dataset curated by retrieving common visual metaphors from real comic datasets such as COMICS \cite{iyyer2017amazing}\cite{chen2021computational} and Manga109\cite{narita2017sketch,matsui2017sketch}. 


==> 5_Results.tex <==
%%% Results and Discussion
%% Summarize any testing or user feedback



% \section{Generated Example with Customization}

% \section{ Experiments }
% \vspace{-0.25cm}
We designed structure refinement layers through VNG and mapped the categories to curves that express narrative-arc to improve action selection for creating content. And another refinement layer employed comic transitions to increase visual variety on panels. Moreover, we applied two extension layers to add richness to image content, Which led to showcases for sample layers.

We first compared generated sequences based on a narrative arc decided by VGN or sequences generated freely. This showcases aims to compare the content differences caused by following the narrative arc. The second part displayed the changes led by the underlying rules applied when constructing content. In other words, this aims to show the possibility of altering the constructing layer to influence content details. Besides the overall structure and component of panels, we also wanted to test the comic sequence's potential by modifying the links between panels. The third part showed the flexibility in controlling the discourse affected by the inter-panel adjustment. The fourth part showed the possibility of extending the generator to enhance the richness of content expression.



% \subsection{Grammar Layer and Action Selection Based on Narrative Arcs}
\subsection{Grammar Layer and Action Selection Based on Narrative Arcs}
% \vspace{-0.25cm}
% In the first experiment, we compared generated sequences based on a narrative arc decided by VGN or sequences or generated freely in the first experiment.

Our first two refinement layers implement the five categories of VGN and expand the center-embedded structure through probability for the whole comic panel. Then, according to the usages that the categories suggested, we mapped the categories to stages in narrative arcs. Then the action candidates that in our dataset utilized the activation and deactivation concept to get a corresponding coordinate in the Circumplex model, figure \ref{affect}. The coordinate implies whether an action raises tensions or drops tensions.

% The stages are denoted by the formula [1], which only be used to compares the changes between narrative stages, such as the climate supposed to have a higher tension value than the rising action. 


Therefore, the expanded narrative grammar tree basically decides how the story looks in the generated comic sequence. The table\ref{grammar_layer_and_arc} shows the results of whether the grammar and narrative arc layer is on or off.
		
\begin{table}
% \vspace*{-4mm}
\centering
\begin{tabular}{|p{1.5cm}|p{6cm}|p{2.5cm}|}
    \hline
    Settings & Layer: Narrative Grammar and Narrative Arc & Narrative Trend\\
    \hline
    % 0 & 3& 8& 0\\
    % \hline    
   with
    &\includegraphics[width = \linewidth]{Images/grammar_yes_1.PNG}
    &\includegraphics[width = \linewidth]{Images/grammar_yes_1_chart.png}\\
    \hline     
   without
    &\includegraphics[width = \linewidth]{Images/grammar_no_2_main.png}
    &\includegraphics[width = \linewidth]{Images/grammar_no_2_chart.png}\\
    \hline     
%   with
%     &\includegraphics[width = \linewidth]{Images/grammar_yes_2.png}
%     &\includegraphics[width = \linewidth]{Images/grammar_yes_2_chart.png}\\
%     \hline     
%   without
%     &\includegraphics[width = \linewidth]{Images/grammar_no_1_2.PNG}
%     &\includegraphics[width = \linewidth]{Images/grammar_no_1_chart.png}\\
%     \hline     


\end{tabular}
    \caption{
    \label{grammar_layer_and_arc} \small{Examples of with or without narrative grammar and narrative structures.}
    }
% \vspace*{-6mm}
\end{table}
The sequence with the narrative-arc layer suggests that the action selection follows a usual pattern. The action has higher tension such as collide and run showed up in peak and then tension relieved by more relaxed actions. And both the action of the characters follow the trend of the tension curve. On the contrary, the characters' action selection becomes rather arbitrary in the sequence without refining the narrative-arc layer. Even in the story peak, the characters take relaxed actions.

\subsection{Action relations network}
% \subsection{Action relations network}
% \vspace{-0.25cm}
The next refinement layer implements are action-reaction relation network of possible actions. For example, the "fall" happens after "jump" or "fly," "dizzy" happens after "collide," and so on. The table \ref{action_net_layer} suggests the results where the action relation network was on or off.
\begin{table}
% \vspace*{-4mm}
\centering
\begin{tabular}{|p{1.5cm}|p{6cm}|}
    \hline
    Settings & Layer: Action Relations Network Layer \\
    \hline
    % 0 & 3& 8& 0\\
    % \hline    
   with
    &\includegraphics[width = \linewidth]{Images/action_yes.PNG}\\
    \hline     
   without
    &\includegraphics[width = \linewidth]{Images/action_no.PNG}\\
    \hline     

\end{tabular}
    \caption{
    \label{action_net_layer} \small{Examples of with or without action relation network.}
    }
% \vspace*{-6mm}    
\end{table}
The sequence with the action relation network can easily link the panel with a continuous story, whereas the other can not. In the former, the blue character "collide" something, so it becomes "angry" and then "dizzy The pink character "fly" and then "falls." After that, it is "shocked" and then takes "a rest." On the contrary, characters in the later sequence select actions randomly.
% \vspace{-0.25cm}


% \subsection{Transition layer}
\subsection{Transition layer}
% \vspace{-0.25cm}
The transition refinement layer uses the transitions to modify the story presentation of the comic sequence. For example, in the table \ref{transition_layer}, the sequence linked by [Aspect, Action, Scene] transitions, adjusted the image's composition, modifies the chosen actions, and transports a significant space. 
The view angle changes make the story a bit more interesting. The modification makes the story seem to be interpreted as two characters meeting in a garden, and one suddenly leaves the place. When the other follows the character, it saw the character sit in the forest. 
\begin{table}
% \vspace*{-4mm}
\centering
\begin{tabular}{|p{1.5cm}|p{6cm}|}
    \hline
    Settings & Layer: Transition layer \\
    \hline
    % 0 & 3& 8& 0\\
    % \hline    
   with
    &\includegraphics[width = \linewidth]{Images/transition_yes.PNG}\\
    \hline
   transition sequence
    &[Aspect-to-Aspect, Action-to-Action, Scene-to-Scene]\\
    \hline      
   without
    &\includegraphics[width = \linewidth]{Images/action_yes.PNG}\\
    \hline     

\end{tabular}
    \caption{
    \label{transition_layer} \small{Examples of with or without transition network.}
    }
% \vspace*{-6mm}    
\end{table}
% \subsection{Customize layers}
\subsection{Customize layers}
% \vspace{-0.25cm}
The final two refinement layers are the cases that extend the generator with either image set or functions. The textbox layer provides three types of text balloon where the sharpness degree of ballon's edge help to emphasize the emotion of characters. The action with higher activation scores will be pairing the sharp ballon when the mild action will be paired with the normal talking ballon. Furthermore, the shapes present whether the character is talking or thinking. The display layer implemented the function that flips the display flag of characters on or off by probability. In the last two panels, as the blue character's display flag was turned off, the whole sequence then shows a story that two characters flying together, but one disappeared eventually. Both of the extended layers enrich the image content and add more detail to the presented story. The results are in table \ref{addtional_layer}  
\begin{table}
% \vspace*{-4mm}
\centering
\begin{tabular}{|p{1.5cm}|p{6cm}|}
    \hline
    Settings &  \\
    \hline
    % 0 & 3& 8& 0\\
    % \hline    
   Textbox layer
    &\includegraphics[width= \linewidth]{Images/text_sample_5.PNG}\\
    \hline     
    
   Display layer
    &\includegraphics[width = \linewidth]{Images/text_sample_2.PNG}\\
    \hline     

\end{tabular}
    \caption{
    \label{addtional_layer} \small{Examples that apply additional refinement layers }
    }
% \vspace*{-6mm}    
\end{table}

\subsection{Story layers}
We used short story text as a content reference in our final customized layer. Our model didn't equip language processing functions, so this layer starts from "assertions": the proceed triples from the narrative representation model--Rensa. The sample story text is below. and the assertions are in table \ref{assertions}.


\{A and B are in the forest. A has B's Apple. B is angry. B enter the scene.\}

As the table \ref{assertions} shows, some links between character, relation, and location are created. And then, the generator modifies the content according to the links. It selects performable actions from the linked action pool. For example, the relation "has" is related to actions like eating and drinking; and the action "angry" links to other action labels such as crying and dizziness. The results are in table \ref{story_layer}.

\begin{table}
% \vspace*{-4mm}
\centering
\begin{tabular}{|p{1.5cm}|p{3cm}|p{1.5cm}|p{1.5cm}|p{4cm}|}
    \hline
    l &  relation & r & r\_owner & links\\
    \hline
    \{A, B\} & \{location\_on\} & \{forest\} & \{\} & \{forest\} \\
    \hline
    \{A\} & \{has\} & \{apple\} & \{B\} & \{eat, drink\} \\
    \hline
    \{B\} & \{action\} & \{angry\} &\{\} & \{angry, dizzy, cry\} \\
    \hline
    \{B\} & \{action\} & \{enter\} &\{\} & \{run, collide\} \\
    % 0 & 3& 8& 0\\
    % \hline    
    \hline     

\end{tabular}
    \caption{
    \label{assertions} \small{Examples that apply short story text as reference.}
    }
% \vspace*{-6mm}    
\end{table}

The example gives a complete story that we can interpret as follows: the two characters are in the forest, and are both eating. Then after one of them finished its apple, it took the other's apple. So, the other character became angry. Then the first character ran, and the other character chased it. Because the content was created depending on the links between story text and links between existing actions in the dataset, it will follow the story flow. 


\begin{table}
% \vspace*{-4mm}
\centering
\begin{tabular}{|p{1.5cm}|p{6cm}|}
    \hline
    Settings &  \\
    \hline
    % 0 & 3& 8& 0\\
    % \hline    
   Story layer
    &\includegraphics[width= \linewidth]{Images/story_example.png}\\
    \hline     

\end{tabular}
    \caption{
    \label{story_layer} \small{Examples that apply additional refinement layers }
    }
% \vspace*{-6mm}    
\end{table}

==> 6_Limitations.tex <==
The system we proposed has some limitations and unsolved issues:\\

1. Although the separation of background and foreground makes user selection convenient and helps partial redraw, it reduces the interaction between the scene and characters, where characters can perform richer actions and make the elements in the overall design usually relate to each other and the whole artwork. \\

2. While we employed emoji and common comic symbols to represent character actions and narratives, the diffusion models can generate the whole image with differences in details. In this paper, we tried to bring authors into the generating process instead of relying on all the AI results. The balance between entirely generated images and human-in-loop generation is worth more discussion. \\

3. The flexibility of narrative elements: although we make significant efforts to bring abstract narrative theories into the generating process, the richness of narrative and the diversity of story content are limited. Integrating this system with powerful language models could bring the richness of the story. \\



==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto
